A Novel Approach to Identify Security Controls in Source Code

Secure by Design has become the mainstream development approach ensuring that software systems are not vulnerable to cyberattacks. Architectural security controls need to be carefully monitored over the software development life cycle to avoid critical design flaws. Unfortunately, functional requirements usually get in the way of the security features, and the development team may not correctly address critical security requirements. Identifying tactic-related code pieces in a software project enables an efficient review of the security controls' implementation as well as a resilient software architecture. This paper enumerates a comprehensive list of commonly used security controls and creates a dataset for each one of them by pulling related and unrelated code snippets from the open API of the StackOverflow question and answer platform. It uses the state-of-the-art NLP technique Bidirectional Encoder Representations from Transformers (BERT) and the Tactic Detector from our prior work to show that code pieces that implement security controls could be identified with high confidence. The results show that our model trained on tactic-related and unrelated code snippets derived from StackOverflow is able to identify tactic-related code pieces with F-Measure values above 0.9.

==> Temp.tex <==
\section{Methodology}

\subsection{Detecting Tactics in Source Code}

\subsection{Data Collection Approach}
Why stack overflow?

How related samples were created?

Dataset was created by collecting Stack Overflow questions relevant to the tactic. We used the /search/advanced api to fetch the questions. This api takes a free form text parameter and returns a list of questions. We used a query related to the tactic that gave us the maximum number of questions as the text parameter. For example, for tactic Advanced Encryption Standard we used "aes" as the text parameter. Stack Overflow matches this parameter with all question properties and returns the relevant questions. The text parameter used for tactics can be found in table-n.

How unrelated samples were created?

Unrelated samples were created from a set of 50000 questions with 'java' tag. Just searching for 'java' will ensure that the questions are general and not biased to anything in particular. We also ensured that the related and unrelated questions did not have any tag in common with the exception of 'java'.

Once the related and unrelated samples were collected, we merged them to create balanced dataset of 300 samples for each tactic.

The code snippets were preprocessed by removing punctuation, removing language(java) related keywords, splitting camelcase words into separate words, removing stop words and numbers and finally converting the whole snippet to lower case.
\subsection{Algorithm}

\subsection{Evaluation}


